Ultra-fine Entity Typing with Indirect Supervision from Natural Language Inference

The task of ultra-fine entity typing (UFET) seeks to predict diverse and free-form words or phrases that describe the appropriate types of entities mentioned in sentences. A key challenge for this task lies in the large amount of types and the scarcity of annotated data per type. Existing systems formulate the task as a multi-way classification problem and train directly or distantly supervised classifiers. This causes two issues: (i) the classifiers do not capture the type semantics since types are often converted into indices; (ii) systems developed in this way are limited to predicting within a pre-defined type set, and often fall short of generalizing to types that are rarely seen or unseen in training. This work presents LITE, a new approach that formulates entity typing as a natural language inference (NLI) problem, making use of (i) the indirect supervision from NLI to infer type information meaningfully represented as textual hypotheses and alleviate the data scarcity issue, as well as (ii) a learning-to-rank objective to avoid the pre-defining of a type set. Experiments show that, with limited training data, LITE obtains state-of-the-art performance on the UFET task. In addition, LITE demonstrates its strong generalizability, by not only yielding best results on other fine-grained entity typing benchmarks, more importantly, a pre-trained LITE system works well on new data containing unseen types.

==> sections/exp_archive.tex <==
\label{sec:experiments}

In this section, we present the experimental evaluation for \modelname framework, based on both UFET (\Cref{ssec:ultra}) and traditional (less) fine-grained entity typing tasks (\Cref{ssec:fine}). In addition, we also conduct comprehensive ablation studies to understand the effectiveness of the incorporated techniques(\Cref{sec:analysis}). 


\subsection{Ultra-Fine Entity Typing}\label{ssec:ultra}
We use the UFET benchmark created by \citet{choi-etal-2018-ultra} for evaluation. This data consists of two parts. (i) Human-labeled data (L): 5,994 instances split into train/dev/test by 1:1:1 (1998 for each); (ii) Distant supervision data (D): 5.2M data automatically labeled by linking entity to KB, and 20M data generated by headword extraction.


% Its whole labeling space contains 10,331 types within which there are 9 general types, 121 fine-grained types and 10,201 ultra-fine types. The full dataset consists of 5,994 human annotated data, \muhao{+splits}.
% It also comes with 5.2M data automatically labeled by linking entity to KB as well as 20M data generated by headword extraction. Such automatically generated data serve as the distant supervision for training. 


\subsubsection{Experimental Settings} 


\stitle{Training Data} In our approach, the supervision can come from the M\textbf{NLI} data (NLI), \textbf{d}istant supervision data (D) and the human-\textbf{l}abeled data (L). Therefore, we investigate the best combination of training data by exploring the following different training pipelines:

% In prior studies, training data for this benchmark, as mentioned before, involves sources of distant supervision data and human annotated data \muhao{+citations}. We accordingly adopt four variants of \modelname to compare with baseline methods that follow different training settings involving such augmented training data: 

\begin{itemize}[leftmargin=1em]
\setlength\itemsep{0em}
    \item \modelname\textsubscript{NLI}: Pretrain on MNLI, then predict directly, without any tuning on D or L;
    \item \modelname\textsubscript{NLI+L}: Pretrain on MNLI, then fine-tune on L;
    \item \modelname\textsubscript{D+L}: Pretrain on D, then fine-tune on L;
    \item \modelname\textsubscript{NLI+D+L}: First pretrain on MNLI, then on D, finally fine-tune on L.
    % \item \modelname\textsubscript{NLI/D$^+$/L}: It follows the training pipeline of \modelname\textsubscript{NLI/D/L} except that we extend D with extra distant supervision data generated by BERT masked language model \cite{Dai2021UltraFineET}. The enlarged distant supervision data is denoted as ``D$^+$''.
    
    % \wenpeng{Since distant supervision doesn't help for your system, it doesn't make sense to report an extended distant supervision data performance}
\end{itemize} 

\stitle{Model Configurations} Our system is first initialized by the RoBERTa-large \footnote{\url{https://huggingface.co/roberta-large}} and AdamW  \cite{loshchilov2018fixing} is used to optimize the model. The hyper-parameters as well as the output threshold are tuned on the dev set: batch size 16, pre-training learning rate 1e-6,  fine-tuning learning rate  5e-6, margin $\gamma$=0.1 and $\lambda$=0.05.

% , are chosen from 0 to 0.4 with a step of 0.1. The hyper-parameter $\lambda$ for controlling the influence of dependency modeling are chosen from 0 to 0.5 with a step of 0.05. Accordingly,  $\gamma$=0.1 and $\lambda$=0.05 are selected for the reported \modelname performances. 

The pre-training epochs are limited to 5 which is enough considering the large size of the pre-training data. The fine-tuning epochs are limited to 2,100; models are evaluated every 30 epochs on dev and the best model is kept to conduct inference on test. 

\stitle{Baselines} We compare our model with the following strong baselines. Except for LRN which is merely trained on the human annotated data, all the other baselines incorporate the distant supervision data as extra training resource. 

\begin{itemize}[leftmargin=1em]
\setlength\itemsep{0em}
    \item \textbf{UFET} \cite{choi-etal-2018-ultra} represents words by GloVe \cite{pennington-etal-2014-glove} embeddings and captures the semantic information of sentence, entity as well as labels by a bi-LSTM and a character-level CNN. It also learns a type label embedding matrix to do inner product with the context and mention representation for classification. 
    \item \textbf{LabelGCN} \cite{xiong-etal-2019-imposing} improves UEFT by stacking a graph convolution layer on the top to capture the latent label dependency. 
    \item \textbf{LDET} \cite{onoe-durrett-2019-learning} applies ELMo \cite{Peters:2018} embeddings for word representation and adopts LSTM for its sentence and mention encoders. Similar to UFET, it learns a matrix to compute inner product with each input representation for classification. Besides, LDET also trains a filter and relabeler to fix the label inconsistency in the distant supervision training data. 
    \item \textbf{BOX4Types} \cite{Onoe2021ModelingFE} introduces box embeddings to handle with the type dependency problems. It uses BERT-Large-uncased \cite{devlin-etal-2019-bert} as the backbone and projects the hidden classification vector to a hyper-rectangular(box) space. Each type from the label space is also dedicated to a box and the classification is fulfilled by computing the intersection of input representation box and type boxes. 
    \item \textbf{LRN} \cite{liu2021finegrained} encodes the context and entity with BERT-base-uncased. Then two LSTM-based auto-regression network captures the context-label relation and the label-label relation via attention mechanisms respectively in order to generate labels. They simultaneously construct bipartite graphs for sentence tokens, entities and generated labels to do relation reasoning and predict more labels.
    \item \textbf{MLMET} \cite{Dai2021UltraFineET} obtains extra supervision from labels generated by BERT Masked Language Model. Their typing model uses BERT-base-cased\footnote{According to their paper, BERT-base-cased outperforms BERT-large and RoBERTa models} as the encoder. The input sentence is formatted as ``[CLS token] sentence [SEP token] entity mention [SEP token]'' and the hidden vector of [CLS token] goes through a linear classification layer to generate the probability of each type.
    \item \textbf{RoBERTa} \cite{liu2019roberta} is added for studying the effectiveness of introducing NLI to this task. Here we adopt the same typing model of MLMET and include both of distant supervision data and human annotated data to achieve its best performance. 
\end{itemize} 

\subsubsection{Results}\label{ssec:ultraRes} 
\input{tables/result}
Following prior studies ~\cite{choi-etal-2018-ultra,onoe-durrett-2019-learning,Dai2021UltraFineET}, we evaluate the loose macro-averaged precision, recall and F-1 on different training settings. 

\stitle{Overall Performance} The results for \modelname with taxonomic statement template (i.e.`` \textit{[ENTITY]} is a \textit{[LABEL]}'') is reported in \Cref{tab:res}. As shown in the table, \modelname\textsubscript{NLI+L} demonstrates state-of-the-art over other baselines, outperforming the existing best approach MLMET \cite{Dai2021UltraFineET} with 1.5\% absolute improvement on F-1 score. The results by \modelname series improve RoBERTa-large baseline method by at least 3.4\% absolute F-1 score, showing that incorporating the inference ability of NLI has better performance than fine-tuning a classification task on pretrained language model. 

For the different training data settings of \modelname, the performance of \modelname\textsubscript{NLI} indicates that simply training the language model on MNLI cannot capture the sentences and type descriptions well. Training with typing data endows the model with ability to distinguish between correct and false type descriptions. \bangzheng{\modelname\textsubscript{D+L}}

In addition, it is noteworthy that \modelname\textsubscript{NLI+L} is trained on only 2k human-annotated data to obtain the best performance over other settings whose training set extends to millions of data samples. Adding distant supervision data even leads to a drop of 2.3\% absolute score in F-1. \modelname\textsubscript{LM-aug} appends MLMET generated data to \modelname\textsubscript{Distant} to get a marginal improvement but still get worse performance than  \modelname\textsubscript{w/o aug}. These results demonstrate that the training data source will affect the typing performance.


\input{tables/trainData}

\stitle{Effect of Training Data}
From our observation, the automatically generated training data is more noisy than human annotated samples. This is also verified by \cite{onoe-durrett-2019-learning} in their paper. \Cref{tab:dataSource} lists some frequent and typical problems for the entity linking and head-word extraction data. The noisy labels in entity linking data mainly consist of unrelated type words. For example, in sample (a), entity \textit{Conneticut} is here labeled as \textit{author}, \textit{cemetery} and \textit{person}. Meanwhile, the head-word extraction can result in incomplete type words and therefore generates incorrect type labels. For the example (d), entity \textit{hash brown} is labeled as \textit{brown}, turning the concept of food into color. Another typical problem is that, the pattern-based extraction method is short in capturing the semantics. In the example (f), \textit{number} is extracted as the type for \textit{a number of short stories} because of the preposition ``of''. 

Another reason for the performance drop in \modelname\textsubscript{Distant} and \modelname\textsubscript{LM-aug} is the incomplete typing labels provided by the distant supervision data. This is common for both of the entity linking data and head word extraction data. For example, example (d) and (g) are about the entity ``film'' where the label words are correct. However, in the human annotated data, entity ``film'' will probably be labeled as (``film'', ``art'',  ``movie'', ``show'', ``entertainment'', ``creation''). In this situation, the unlabeled (``movie'', ``show'', ``entertainment'', ``creation'') can be selected by the negative sampling process of \modelname and therefore influence the performance. Incorporating Labels generated by language model(MLMET) can solve this problem to some extent but is still not perfect. For instance, in ``3 Ninjas Kick Back is a 1994 American sequel to the film 3 Ninjas.'', entity ``film'' is labeled by BERT as (``sequel'', ``\st{title}'', ``film'', ``movie'', ``\st{original}'', ``\st{game}'', ``series'', ``\st{feature}'', ``\st{classic}'', ``\st{starring}'') where incorrect labels are stroke through.

\stitle{Few-shot Prediction} Since there is non-overlapping type coverage of the human annotated train set and test set, we investigate on the \modelname\textsubscript{w/o aug} performance breakdown considering the frequency of test set labels in the train set. \Cref{fig:fewShot} shows the results where the strongest baseline, MLMET, is added for comparison even if it is trained with LM-augmented data, distant supervision data and human annotated data which provide abundant training resources\footnote{Though 52 out of 549 zero-shot labels are still missing in their training data}. 

It is expected that the performance on more frequent labels are better than on rare labels because of the ampler training cases. Nevertheless, \modelname\textsubscript{w/o aug} outperforms MLMET on all the listed frequency of labels which reveals the strong few-shot prediction performance of our model. In addition, on the extremely challenging zero-shot labels, \modelname\textsubscript{w/o aug} drastically improves the F-1 score from 19.3\% to 33.1\%. Given these facts can we conclude that the template-based type description is effective for transferring the inference ability of NLI from training data to labels. 

\begin{figure}[ht]
\includegraphics[width=7.6cm]{figures/fewShot.pdf}
\caption{Few Shot}
\label{fig:fewShot}
\end{figure}

\stitle{Ablation Study} 
To understand how dependency modeling influence the typing results, we investigate the performance breakdown  of \modelname\textsubscript{w/o aug} of different label specificity on the test set. In \Cref{tab:breakdown}, label dependency modeling mostly improves \modelname\textsubscript{w/o aug} on the fine-grained types by 2.6\% F-1 score. This is because fine-grained labels, as the most infrequent labels, only takes up 12.1\% of the label occurrences in the human annotated train set. During the dependency modeling phase, type descriptions of ultra-fine grained labels, which in total take up 70.1\% of the training labels, therefore provide indirect supervision to these infrequent labels. General labels also benefit from this mechanism with 2.6\% absolute improvement.

\Cref{tab:ablation} reveals how template choices affect the typing performance. It is obvious that taxonomic statement beats the other two under all of the three training settings. The contextual explanation template yields close but worse results while the label substitution leads to noticeable F-1 drop. Here we provide some detailed case study for this phenomenon.

\input{tables/breakdown}
\input{tables/ablation} 

\stitle{Case Study}
We present a case study with three representative cases for \modelname\textsubscript{Direct} with three templates (\Cref{tab:caseStudy}). In the first example, Taxonomic Statement and Contextual Explanation based models correctly predict part of the human annotation and labeled \textit{soft eye shields} with \textit{covering} and \textit{defense} respectively, which is reasonable from human's recognition. However, Label Substitution presents trivial label \textit{item} and wrong label \textit{tissue}. For the second example, three template based models correctly types the entity with the words from human annotated labels. Their false positive labels such as \textit{play}, \textit{film} and \textit{entertainment} are compatible with the given context. Nevertheless, none of them can predict a label other than \textit{person} in the third sentence. From human's perspective, it is natural to assume \textit{he} is an \textit{economist} or an \textit{administrator} while \modelname failed to capture such information.  




\subsection{Fine-Grained Entity Typing}\label{ssec:fine}

\muhao{Can ``tranditional'' be changed to something else? E.g., ``Less''?}

In this section, we evaluate \modelname on Ontonotes \cite{gillick2014context} as well as FIGER \cite{ling2012fine}.  

\stitle{Ontonotes} For the OntoNotes data set, we use the version provided by \citet{choi-etal-2018-ultra}, which includes 3.4M automatically labeled data for training and 11k manually annotated samples split into 8k for development set and 2k for test set. Its label space consists of 89 type words in canonical form. We compare \modelname with 4 following approaches: UFET \cite{choi-etal-2018-ultra}, LDET\cite{onoe-durrett-2019-learning}, DSAM\cite{9305269} and MLMET\cite{Dai2021UltraFineET}. DSAM utilizes a diversified semantic attention mechanism to capture both context-level and mention-level information. 

In the label space of OntoNotes, there is a word \textit{other} that produces meaningless type descriptions for \modelname. Though its descendant types are meaningful words, \textit{other} sometimes appears alone to label the entity mentions that is difficult to be described as the other 88 words. For example, entity \textit{Friday} is therefore labeled as a single \textit{other}. To alleviate this problem, we modified \modelname to produce a single \textit{other} if no type descriptions is scored over the threshold described in \Cref{ssec:inf}.

\stitle{FIGER} The FIGER data set contains 2M data samples labeled with 112 types. The development set and test set includes 1,000 and 562 samples respectively. Within its label space, 82 type words have a dependency relation with their ancestor or descendant types while the other 30 types are uncategorized free-form words. 

For this benchmark, we compare \modelname with the following methods: ERNIE \cite{zhang-etal-2019-ernie}, WKLM \cite{Xiong2020Pretrained}, DSAM \cite{9305269} and K-ADAPTER \cite{DBLP:journals/corr/abs-2002-01808}. ERNIE takes entity embeddings pre-trained from knowledge graphs as inputs to the Transformer so as to capture the entity relations. Similarly, K-ADAPTER introduces a plug-in neural adaptor that infuse factual and linguistic knowledge into the pre-trained language model. WKLM replaces the entity mention in the sentence with different words of same type for knowledge learning.

\stitle{Evaluation} Following the aforementioned baselines on Ontonotes and FIGER, we report strict accuracy, macro-averaged F-1 and micro averaged F-1. Taxonomic statement template is chosen for both task and output threshold is selected for best performance on development sets.
\input{tables/ontoResult}
\input{tables/figerResult}
% \bangzheng{Ongoing Results}

According to the results in \Cref{tab:ontoRes}, the performance of \modelname on OntoNotes closely matches the best method MLMET considering the accuracy and Micro-F1. However, the Macro-F1 score of \modelname is noticeably lower. From our observation, ambiguity of the type word \textit{other} is the main reason. Besides of the situation mentioned above that some un-categorizable entity may be labeled as \textit{other}, there are number of test samples where  \textit{/other} coexists with labels such as \textit{/organization} and \textit{/company}. In such case, \modelname is unable to generate \textit{other}. 

\Cref{tab:figerRes} shows that \modelname achieves competitive performance on FIGER dataset. Unlike the UFET task, \modelname marginally improves the micro-F1 score. We think this is because these traditional fine-grained entity typing data sets heavily focus on coarse-grained types. Since it takes only 10 types to cover more than 80 percent of all the labels of them \cite{choi-etal-2018-ultra} , our objective at ranking makes little differences. Besides, those general and summary type words yield poor type descriptions that make the inference ability of NLI less beneficial.


\subsection{Analysis}\label{sec:analysis}

==> tables/ablation.tex <==

                                                % comparison between templates
\begin{table}[t]
\small
\begin{tabular}{llll}
\toprule
Templates of \modelnamets\textsubscript{NLI+L}               & \multicolumn{1}{c}{P}    & R                        & F-1                      \\ \midrule
Taxonomic Statement     & 52.4        & 48.9         & 50.6                     \\
Contextual Explanation  & 50.8        & 49.7         & 50.2                     \\
Label Substitution      & 45.2        & 52.1         & 48.4                     \\
\bottomrule
\end{tabular}
%\vspace{-0.5em}
\caption{\label{tab:ablation}}
\end{table}


                                                % original
% \begin{table}[t]
% \small
% \begin{tabular}{llll}
% \toprule
% % & \multicolumn{3}{c}{Test Set}                                                   \\ \cmidrule(l){2-4} 
% Model               & \multicolumn{1}{c}{P}    & R                        & F-1                      \\ \midrule
% \modelnamets\textsubscript{w/o aug}    & 54.5                     & 46.9                     & 50.4                     \\
% % -{\scriptsize w/o dependency modeling}     & 52.1                     & 47.5                     & 49.7                     \\
% -{\scriptsize contextual explanation template} & 50.8           & 49.7            & 50.2                        \\
% -{\scriptsize label substitution template}     & 51.0        & 46.4         & 48.6                     \\ \midrule
% \modelnamets\textsubscript{Distant}  & \multicolumn{1}{r}{50.9} & \multicolumn{1}{r}{45.9} & \multicolumn{1}{r}{48.3} \\
% % -{\scriptsize w/o dependency modeling}     & 49.2                     & 46.7                     & 48.0                     \\
% -{\scriptsize contextual explanation template} & 49.7        & 46.2         & 47.9                        \\
% -{\scriptsize label substitution template}     & 49.2        & 46.1         & 47.6                     \\ \midrule
% \modelnamets\textsubscript{LM-aug} & \multicolumn{1}{r}{51.4} & \multicolumn{1}{r}{46.8} & \multicolumn{1}{r}{49.0}   \\
% % -{\scriptsize w/o dependency modeling}     & 50.3                     & 46.9            & 48.5             \\
% -{\scriptsize contextual explanation template} & 50.6        & 47.1            & 48.8             \\
% -{\scriptsize label substitution template}     & 50.1        & 46.8            & 48.4             \\
% \bottomrule
% \end{tabular}
% \caption{\label{tab:ablation}}
% \end{table}

==> tables/caseStudy_archive.tex <==
\begin{table}[]
\def\arraystretch{1.2}
\scriptsize
\begin{tabular}{l|p{0.5\linewidth}}
\hline
Sentence               & \textbf{Soft eye shields} are placed on the baby to protect their eyes from damage that may lead to retinopathy due to the bili lights. \\
\cline{2-2}
Human                  & device, shield, object, guard, protection, defender, shade, object                                                             \\
\cline{2-2}
Taxonomic Statement    & device, shield, object,  protection, covering                                                                                  \\
\cline{2-2}
Contextual Explanation & shield, object, protection, safeguard, defense                                                                                 \\
\cline{2-2}
Label Substitution     & treatment, tissue,  safety glasses, item, device, shield, object                                                               \\ \hline
Sentence               & Queen Mary, the Queen Mother, came to see \textbf{it}, and after the performance asked Cotes where he found those wonderful actors. \\
\cline{2-2}
Human                  & show, performance, event                                                                                                       \\
\cline{2-2}
Taxonomic Statement    & show, performance, event, movie, film, play                                                                                    \\
\cline{2-2}
Contextual Explanation & show, performance, event, object, play                                                                                         \\
\cline{2-2}
Label Substitution     & show, performance, event, movie, film, play, act, entertainment, opera, concert, theater                                       \\ \hline
Sentence               & However, the sustained growth in labour productivity should still provide an alleviating effect, \textbf{he} added.                  \\
\cline{2-2}
Human                  & administrator, economist, leader, person                                                                                       \\
\cline{2-2}
Taxonomic Statement    & person                                                                                                                         \\
\cline{2-2}
Contextual Explanation & person                                                                                                                         \\
\cline{2-2}
Label Substitution     & person                                                                                                                         \\ \hline
\end{tabular}
\caption{\label{tab:caseStudy}}
\end{table}

==> tables/fewShot.tex <==
                % LITE vs MLMET only on F-1

\begin{table}[t]
\small
\begin{tabular}{@{}l|cccc}
\toprule
        & \multicolumn{4}{c}{F-1 on different Label Frequency}                 \\ \cmidrule(l){2-5} 
Model  & \multicolumn{1}{l}{\scriptsize{0 shot}} & \multicolumn{1}{l}{\scriptsize{1$\sim$5 shot}} & \multicolumn{1}{l}{\scriptsize{6-10 shot}} & \multicolumn{1}{l}{\scriptsize{11$\sim$100 shot}} \\ \midrule
MLMET       & 19.3     & 27.8     & 32.7     & 44.0                                \\
\modelname   & 33.1    & 34.4     & 38.3     & 45.3                                \\ \bottomrule
\end{tabular}
\caption{Few shot Result}
\label{tab:fewShot}
\end{table}

                    % Original lite + lite w/o depend + MLMET
% \begin{table*}[t]
% \small
% \begin{tabular}{@{}l|lll|lll|lll}
% \toprule
%                       & \multicolumn{3}{c|}{\modelname} & \multicolumn{3}{c|}{\begin{tabular}[c]{@{}c@{}}\modelname\scriptsize{-w/o dependency}\end{tabular}} & \multicolumn{3}{c}{MLMET} \\ \cmidrule(l){2-10} 
%  \small{Test Set Labels in Train Set}     & P        & R        & F-1      & P                          & R                          & F-1                        & P       & R       & F-1    \\ \midrule
% 0-shot labels            & 62.55    & 22.5     & 33.10     & 42.48                      & 27.26                      & 33.21                      & 68.0    & 11.24   & 19.30   \\
% 1$\sim$5-shot labels     & 43.80    & 28.34    & 34.42    & 37.7                       & 32.06                      & 34.65                      & 50.56   & 19.21   & 27.84  \\
% 6$\sim$10-shot labels    & 41.09    & 35.94    & 38.34    & 33.23                      & 39.39                      & 36.05                      & 46.49   & 25.21   & 32.69  \\
% 11$\sim$100-shot labels  & 45.04    & 45.5     & 45.27    & 36.09                      & 52.66                      & 42.83                      & 45.56   & 42.57   & 44.01  \\
% % 101$\sim$759-shot labels & 66.02    & 71.96    & 68.86    & 54.67                      & 84.08                      & 66.26                      & 61.83   & 76.25   & 68.29  \\ 
% \bottomrule
% \end{tabular}
% \caption{\label{tab:fewShot}}
% \end{table*}

                    % LITE vs MLMET
% \begin{table*}[t]
% \small
% \begin{tabular}{@{}l|lll|lll}
% \toprule
%                       & \multicolumn{3}{c|}{\modelname} & \multicolumn{3}{c}{MLMET} \\ \cmidrule(l){2-7} 
%  \small{Labels Frequency}    & P      & R     & F-1    & P       & R       & F-1    \\ \midrule
% 0-shot labels            & 62.55    & 22.5     & 33.10    & 68.0    & 11.24   & 19.30   \\
% 1$\sim$5-shot labels     & 43.80    & 28.34    & 34.42    & 50.56   & 19.21   & 27.84  \\
% 6$\sim$10-shot labels    & 41.09    & 35.94    & 38.34    & 46.49   & 25.21   & 32.69  \\
% 11$\sim$100-shot labels  & 45.04    & 45.5     & 45.27    & 45.56   & 42.57   & 44.01  \\
% \bottomrule
% \end{tabular}
% \caption{\label{tab:fewShot}}
% \end{table*}

                


==> tables/figerResult.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\centering
\scriptsize
\def\arraystretch{1.2}
\begin{tabular}{@{}lrrr@{}}
\toprule
          &      & FIGER &      \\ \cmidrule(l){2-4} 
Model     & Acc                       & Ma-F1                     & Mi-F1 \\ \midrule
ERNIE     & 57.2                     & 75.6                     & 73.4                     \\
WKLM      & 60.2                     & 82.0                     & 77.0                          \\
DASM      & 69.4                     & 83.3                     & 81.5                     \\
K-ADAPTER & 61.8                     & 84.9                     & 80.5                     \\ \midrule
\modelname & 60.6                    & 85.8                     & 80.6                      \\
\bottomrule
\end{tabular}
\caption{\label{tab:figerRes} Results on FIGER}
\end{table}

==> tables/ontoResult.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\centering
\scriptsize
\def\arraystretch{1.2}
\begin{tabular}{@{}lrrr@{}}
\toprule
          & \multicolumn{1}{l}{}    & \multicolumn{1}{c}{OntoNotes} & \multicolumn{1}{l}{}      \\
\cmidrule(l){2-4} 
Model     & Acc                     & Ma-F1                         & Mi-F1                     \\ \midrule
UFET      & 59.5                    & 76.8                          & 71.8                      \\
LDET      & 64.9                    & 84.5                          & 79.2                      \\
DSAM      & 66.1                    & 83.1                          & 78.2                     \\
MLMET     & 67.4                    & 85.4                          & 80.4                     \\ \midrule
\modelname& 62.0                    & 84.5                          & 80.0                      \\ 
\modelname\textsubscript{w/o aug} &65.0	&87.6	                    &83.4                       \\
\bottomrule
\end{tabular}
%\vspace{-0.5em}
\caption{\label{tab:ontoRes}Result on OntoNotes}
\end{table}
